SoK: Security of Cross-chain Bridges: Attack Surfaces, Defenses, and Open Problems

Cross-chain bridges are used to facilitate token and data exchanges across blockchains. Although bridges are becoming increasingly popular, they are still in their infancy and have been attacked multiple times recently, causing significant financial loss. Although there are numerous reports online explaining each of the incidents on cross-chain bridges, they are scattered over the Internet, and there is no work that analyzes the security landscape of cross-chain bridges in a holistic manner. To fill the gap, in this paper, we performed a systematic study of cross-chain bridge security issues. First, we summarize the characteristics of existing cross-chain bridges, including their usages, verification mechanisms, communication models, and three categorizations. Based on these characteristics, we identify 12 potential attack vectors that attackers may exploit. Next, we introduce a taxonomy that categorizes cross-chain attacks in the past two years into 10 distinct types, and then provide explanations for each vulnerability type, accompanied by Solidity code examples. We also discuss existing and potential defenses, as well as open questions and future research directions on cross-chain bridges. We believe that this systematization can shed light on designing and implementing cross-chain bridges with higher security and, more importantly, facilitating future research on building a better cross-chain bridge ecosystem.

==> 3-attack.tex <==
\section{Bridge Attack Surfaces}
\label{sec:vuls}
% This paper summarizes all the major hacks or attacks which caused huge financial losses. Except for the three categories presented in~\secref{sec:taxonomy}, there are some potential vulnerabilities that may open new attack surfaces. We leave a study on these potential vulnerabilities as future work.  

% We illustrate all the possible attacking surfaces of bridges, according to the two types of bridge mechanisms mentioned in \secref{sec:pre}. 
% In particular, the attacking surfaces are classified into xxx types, including 

In this section, we illustrate possible attack surfaces of bridges with 18 specific potential attacks, according to the two bridge models in \secref{sec:pri:mec}. 
In particular, A1, A3, A6, A9, A10, A11, and A12 in \secref{sec:vuls:lm} can also be applied in the Liquidity-Pool-Based model. Moreover, A13, A14, A15, A16, A17, and A18 in \secref{sec:vuls:lp} are also applicable to the Lock-and-Mint; Burn-and-Release model.
\xz{basically, about 13 of them can apply to both models? then, can we just talk about these common ones first, then explain the unique ones?} \mz{make sense}
% \xz{This is a bit confusing; maybe move to the start or the end of Sec. 4} \mz{ok}
% \mz{this section is derived from section 6: potential vulnerabilities in the asiaccs version}
% \xz{3.1/3.2 subsection headers are the two mechenisms, but 3.3/3.4 are the entities, why? seems inconsistent}
\subsection{Lock-and-Mint; Burn-and-Release Model}
\label{sec:vuls:lm}
% We list 12 potential attacks in this mechanism. 

\bheading{A1: Inaccurate deposit.} This attack can happen in step \ding{182} in~\figref{figs:workflow}. Users need to deposit tokens the bridge account. If the bridge account is set with wrong values, the deposited tokens will be lost. Another attack situation is that the related events are incorrect. 

\bheading{A2: Locked liquidity.} This attack can happen in step \ding{182} in~\figref{figs:workflow}. When the assets are transferred to the source blockchain bridge accounts, the tokens will be locked until the wrapped tokens in the destination blockchain are returned. Thus, there will be huge amounts of locked liquidity in the smart contracts which attract attackers extensively. 

\bheading{A3: Mishandling of events.} This attack can happen in step \ding{183} in~\figref{figs:workflow}. Bridges will first fetch and parse the events from the transactions. If these events are handled incorrectly, bridges might perform inappropriate actions, such as sending more money to the users than desired. For example, if a \textit{Deposit} event recording a 10 \textit{ETH} transfer in the source blockchain is mistakenly treated as a 100 \textit{ETH} transfer, bridges will send 100 \textit{ETH} to the user in the destination blockchain.  

\bheading{A4: Problematic mint.} This attack can happen in step \ding{184} in~\figref{figs:workflow}. Once the tokens are locked in the source blockchain, the bridges will take the \textit{Deposit} events as proofs to mint wrapped tokens in the destination blockchain. However, the \textit{Deposit} events can be faked by attackers or used in multiple times to mint more tokens than desired, if the proof is not validated appropriately in the minting process. 

\bheading{A5: Fake burn.} This attack can happen in step \ding{185} in~\figref{figs:workflow}. To get the tokens back in the source blockchain, users should burn the wrapped tokens in the destination blockchain. If there are some permission check issues that allow users to pass the burn, attacks can happen due to the fake burns in which attackers burn nothing but get burn proofs. 

\bheading{A6: Unsent cross-chain messages.} This attack can happen in step \ding{186} in~\figref{figs:workflow}.
The cross-chain bridges rely heavily on the bridge off-chain server (\BOS), who should be responsible for blockchain monitoring, information parsing, and submitting related transactions, to transfer the tokens back to users. Thus, if the related messages are not sent at all, user will not receive their tokens.

\bheading{A7: Incorrect release.} This attack can happen in step \ding{187} in~\figref{figs:workflow}. If the \textit{Burn} event is not generated correctly, there will be problems when releasing original tokens to users. For example, the amount of burnt tokens logged in the event is more than the reality, users can steal money. 

\bheading{A8: Replayed/Unlimited withdraw.} This attack can happen in step \ding{188} in~\figref{figs:workflow}. The release proof needs validation before transferring tokens back to users. However, if the proof can be used multiple times or forged, the withdraw process can go wrong and the money in bridges will be stolen. 

\bheading{A9: Inconsistent transfer.} This attack can happen in step \ding{183} or \ding{186} in~\figref{figs:workflow}.
The root cause is that there are inconsistencies between the cross-chain transactions. Assume a user \AS transfers \textit{ETH} tokens from Ethereum (source blockchain) to BNB (destination blockchain), there are two related transactions (\textit{TxLock} in Ethereum and \textit{TxMint} in BNB). If the amount of transferred token in \textit{TxMint} is incorrect (e.g., less than expected), it is reasonable to doubt that the bridge may be malicious or the smart contracts are vulnerable. 
% If the amount of transferred token in \textit{TxMint} is incorrect (e.g., less than expected), it is reasonable to doubt that the bridge may be malicious and may have launched the incorrect transfer in \textit{TxMint} deliberately. 
% Another similar problem is that the receiver address to obtain minted tokens in \textit{TxMint} is not the same as what the user \AS specifies (\AD). This attack can happen in step \ding{187} in~\figref{figs:workflow}.

\bheading{A10: Single points of failures.} This attack can happen in \BOS in~\figref{figs:workflow}. Bridges have different security levels. For bridges with external verifiers, they can be attacked if enough verifiers are compromised. In particular, the assets in the bridge accounts can be drained or the tokens can be minted without depositing anything. Moreover, the verifiers might be dishonest if the values in the bridges are far more than the values lost as punishments for behaving maliciously. 

% Except for the above attacking surfaces, the bridges themselves can be attackers (e.g., rugpull) or suffer from the current popular DeFi attacks when more functionalities are introduced in the future.

\bheading{A11: Rugpull.} This attack can happen if the bridge itself is the attacker. Rugpulls are scams 
in which the token founders suddenly vanish
and take all the assets with them.
For example, users of Luna Yield that is a farming project on Solana blockchain suffered from the rugpull on 08/19/2021, in which the creators suddenly deleted the website and disappeared~\cite{rugpull-luna}.
Additionally, the investors of a NFT game DApp, BlockVerse, withdrew all the money and disappeared on 01/25/2022~\cite{rugpull-blockverse}.
Users should watch out for the possibility of rugpull in cross-chain bridges, especially that many bridges are invented recently, and they usually attract funds from users at the very beginning when they are created.

\bheading{A12: Existing vulnerabilities in DeFi.} This attack can happen in \CS or \CD in~\figref{figs:workflow}.
DeFi vulnerabilities can also exist in cross-chain bridges. Current cross-chain bridges only support simple DeFi services, which are mainly token transfers and swaps. However, we believe the attacking surface is much larger than the current problems reported in~\secref{sec:taxonomy};
previous well-known DeFi attacks can be applicable, such as the price manipulation attack. 
For example, if the bridge relies on the unstable price oracles,  
which could be maliciously manipulated by the attackers, 
the bridges will suffer from the price manipulation attacks.
Moreover, some popular attacks (e.g., access control) can also happen in the bridge smart contracts. \mz{need revision, make this type a general case}


% \bheading{Cross-chain inconsistencies.} 
% The root cause is that there are inconsistencies between the cross-chain transactions.  
% \begin{packeditemize}
%     \item \textit{Incorrect transfer.} Assume a user \AS transfers \textit{ETH} tokens from Ethereum (source blockchain) to BNB (destination blockchain), there are two related transactions (\textit{TxLock} in Ethereum and \textit{TxMint} in BNB). If the amount of transferred token in \textit{TxMint} is incorrect (e.g., less than expected), it is reasonable to doubt that the bridge may be malicious and may have launched the incorrect transfer in \textit{TxMint} deliberately. Another similar problem is that the receiver address to obtain minted tokens in \textit{TxMint} is not the same as what the user \AS specifies (\AD). In these incorrect transfer cases, the bridge may be malicious.
% \end{packeditemize}

% \bheading{Bridge smart contract bugs.} 
% \begin{packeditemize}
%     \item 
% \end{packeditemize}


% \begin{figure}[!htbp]
% \setlength{\fboxsep}{0pt}%
% \setlength{\fboxrule}{0pt}%
% %\begin{center}
% \tiny
% \centering

% \begin{lstlisting}[language=Solidity]
% contract Bridge {
%   address bridgeAdmin;
%   mapping(address => uint256) balances;
%   uint256 liquidReserves;
  
%   modifier onlyAdmin {
%     require(msg.sender == bridgeAdmin);
%   }

%   constructor(address _bridgeAdmin) {
%     bridgeAdmin = _bridgeAdmin;
%   }
  
%   function changeAdmin(address _newAdmin) public onlyAdmin {
%     bridgeAdmin = _newAdmin;
%   }

%   function addLiquidity(uint256 tokenAmount) public payable {
%     require(balances[msg.sender] >= tokenAmount);
%     uint256 lpTokenAmount = tokenAmount / exchangeRatio();
%     mint(msg.sender, lpTokenAmount);
%     liquidReserves += tokenAmount;
%     emit AddLiquidity(tokenAmount, lpTokenAmount, msg.sender);
%   }

%   function removeLiquidity(uint256 lpTokenAmount) public {
%     uint256 tokenAmountReturn = lpTokenAmount * exchangeRatio();
%     require(liquidReserves >= tokenAmountReturn);
%     burn(msg.sender, lpTokenAmount);
%     liquidReserves -= tokenAmountReturn;
%     emit RemoveLiquidity(tokenAmountReturn, lpTokenAmount, msg.sender);
%   }
% }
% \end{lstlisting}

% \caption{An example of bridge smart contract.}
% \label{figs:bsc}
% % \vspace{-8pt}
% \end{figure}

% \bheading{Bridge smart contract bugs.} We illustrate potential bugs, according to~\figref{figs:bsc} that shows the normal workflow of this mechanism in Solidty code. 
% \begin{packeditemize}
%     \item 
% \end{packeditemize}


\subsection{Liquidity-Pool-Based Model}
\label{sec:vuls:lp}
% We list 7 potential attacks. 
% This type of problems only exist in the liquidity pool based mechanism.
% \vspace{-10pt}
\begin{figure}[!htbp]
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{0pt}%
%\begin{center}
\tiny
\centering

\begin{lstlisting}[language=Solidity]
contract LiquidityPool {
  address bridgeAdmin;
  mapping(address => uint256) balances;
  uint256 liquidReserves;
  
  modifier onlyAdmin {
    require(msg.sender == bridgeAdmin);
  }

  constructor(address _bridgeAdmin) {
    bridgeAdmin = _bridgeAdmin;
  }
  
  function changeAdmin(address _newAdmin) public onlyAdmin {
    bridgeAdmin = _newAdmin;
  }

  function addLiquidity(uint256 tokenAmount) public payable {
    require(balances[msg.sender] >= tokenAmount);
    uint256 lpTokenAmount = tokenAmount / exchangeRatio();
    mint(msg.sender, lpTokenAmount);
    liquidReserves += tokenAmount;
    emit AddLiquidity(tokenAmount, lpTokenAmount, msg.sender);
  }

  function removeLiquidity(uint256 lpTokenAmount) public {
    uint256 tokenAmountReturn = lpTokenAmount * exchangeRatio();
    require(liquidReserves >= tokenAmountReturn);
    burn(msg.sender, lpTokenAmount);
    liquidReserves -= tokenAmountReturn;
    emit RemoveLiquidity(tokenAmountReturn, lpTokenAmount, msg.sender);
  }
}
\end{lstlisting}

\caption{An example of liquidity pool smart contract.}
% Across Protocol https://etherscan.io/address/0x43298f9f91a4545df64748e78a2c777c580573d6#code
\label{figs:lpsc}
% \vspace{-8pt}
\end{figure}

% \bheading{Liquidity pool smart contract bugs.} 
Each liquidity pool is usually related to a smart contract created by the bridge; there will be at least two functions defined for adding and removing liquidity in such contracts. 
% We illustrate potential bugs, according to that 
We show the normal workflow of liquidity pool in~\figref{figs:lpsc}, and use this example to explain the potential bugs. 
\xz{this subsection seem  to be overlapping with A12: existing vuls in Defi} \mz{A12 is a general attack surface, A13-18 are specific attacks}

\bheading{A13: Incorrect initialization.} Bridge accounts will be set as the admin/owner addresses of the liquidity pool during the pool contract creation. If these privileged addresses are initialized with incorrect values in Line 10-11, the total assets in the smart contract can be drained. 

\bheading{A14: Inappropriate function permission.} Similarly, there are some special functions changing the privileged addresses or controlling the contracts, such as killing or pausing the contracts when the caller is admin/owner. If these functions are created with inappropriate permissions in Line 14-15 (e.g., allowing anyone to call them), the contracts will be hacked.

\bheading{A15: Unchecked balance.} To add liquidity to the pools, the liquidity providers should transfer their tokens. If the balance of tokens is not checked in Line 19, attackers can deposit nothing or tokens with less value than the value of returned tokens (e.g., LP tokens). Similarly, there will be problems if balance check is not performed correctly in Line 28.

\bheading{A16: Miscalculated token price.} If the amount of LP tokens is given to the liquidity providers more than desired due to the miscalculated token price in Line 20, the pool will lose money. In particular, the function \textit{exchangeRatio} calculates the token price. Similarly, in the liquidity remove process, if the amount of original tokens returned to the liquidity providers is more than desired in Line 27, there will be financial losses too. 

\bheading{A17: Inconsistent event.} The events will be emitted for off-chain bridge server to monitor, when non-trivial actions happen. For example, \textit{AddLiquidity} event is emitted in Line 23 when the function \textit{addLiquidity} is called. If the \textit{tokenAmount} representing the amount of deposited tokens is wrong, the bridge will get incorrect information and there will be inconsistencies. Similarly, the event \textit{RemoveLiquidity} in Line 31 should be correctly recorded. 

\bheading{A18: Reentrancy.} Reentrancy attack happens when the victim contract call a malicious contract who calls back to the original function in the victim contract, to steal money. In both functions \textit{addLiquidity} and \textit{removeLiquidity}, the reentrancy can occur.


% \bheading{A19: Insufficient liquidity.} This attack can happen in step \ding{174} in~\figref{figs:workflow}. If there is not enough liquidity in the liquidity pool, the cross-chain transactions will not succeed until the liquidity is added. For example, \textit{USDT} liquidity on BSC will be drained faster than Ethereum if there are huge demands of \textit{USDT} on BNB.
% \xz{why this is attack?} \mz{will delete it since it is not real attack}


 % For instance, liquidity of USDT on Binance Smart Chain might be drained faster than ETH due to high demand of USDT usage on BSC. In this case, BSC will have less liquidity to withdraw for users

% not belonging to the cross-chain bridge
% \bheading{High slippage.} This attack can happen in step \ding{174} in~\figref{figs:workflow}. Slippage is the maximum different users would accept in loss during cross-chain token transfers. If the balances of tokens in liquidity pools decrease significantly, the slippage will be very high and the transactions will fail then.


% \subsection{Bridge Off-chain Server}
% Generally, the \BOS go through 5 steps, including fetch event, verify, create transaction, sign, and send, as shown in~\figref{figs:workflow} and~\figref{figs:lp_workflow}.   

% \bheading{Handling events incorrectly.} Bridges will first fetch and parse the events from the transactions. If these events are handled incorrectly, bridges might perform inappropriate actions, such as sending more money to the users than desired. For example, if a \textit{Deposit} event recording a 10 \textit{ETH} transfer in the source blockchain is mistakenly treated as a 100 \textit{ETH} transfer, bridges will send 100 \textit{ETH} to the user in the destination blockchain.  

% \bheading{Unsent cross-chain messages.} 
% The cross-chain bridges rely heavily on the bridge off-chain server (\BOS), who should be responsible for blockchain monitoring, information parsing, and submitting related transactions, to transfer the tokens back to users. Thus, if the related messages are not sent at all, user will not receive their tokens.

% \bheading{Single points of failures.} Bridges have different security levels. For bridges with external verifiers, they can be attacked if enough verifiers are compromised. In particular, the assets in the bridge accounts can be drained or the tokens can be minted without depositing anything. Moreover, the verifiers might be dishonest if the values in the bridges are far more than the values lost as punishments for behaving maliciously. 
% % Thus, the attacking surfaces that could be exploited by attackers mainly are the smart contracts and off-chain server that controls the assets and processes the cross-chain transactions.


% \subsection{Bridge}
% Except for the above attacking surfaces, the bridges themselves can be attackers (e.g., rugpull) or suffer from the current popular DeFi attacks when more functionalities are introduced in the future.

% \bheading{Rugpull.} 
% % DeFi projects attract funds from users at the very beginning
% % when they are created.
% Rugpulls are scams 
% in which the token founders suddenly vanish
% and take all the assets with them.
% For example, users of Luna Yield that is a farming project on Solana blockchain suffered from the rugpull on 08/19/2021, in which the creators suddenly deleted the website and disappeared~\cite{rugpull-luna}.
% Additionally, the investors of a NFT game DApp, BlockVerse, withdrew all the money and disappeared on 01/25/2022~\cite{rugpull-blockverse}.
% % \josh{Remove for another example}
% % \xz{add one or two examples}
% % and leave valueless assets to their users. 
% %  and then take the assets away. 
% % \mz{I removed the types of rugpull}
% Users should watch out for the possibility of rugpull in cross-chain bridges, especially that many bridges are invented recently, and they usually attract funds from users at the very beginning when they are created.

% \bheading{Existing vulnerabilities in DeFi.} 
% DeFi vulnerabilities can also exist in cross-chain bridges. Current cross-chain bridges only support simple DeFi services, which are mainly token transfers and swaps. However, we believe the attacking surface is much larger than the current problems reported in~\secref{sec:taxonomy};
% % and can be extended to 
% previous well-known DeFi attacks can be applicable, such as the price manipulation attack. 
% For example, if the bridge relies on the unstable price oracles,  
% which could be maliciously manipulated by the attackers, 
% the bridges will suffer from the price manipulation attacks.

% original table
% \begin{table*}[t]
%     \centering
%     % \resizebox{0.95\linewidth}{!}{
%     % \scriptsize
%     \footnotesize
%     \begin{tabular}{lllllllll}
%       \toprule
%       Type & Sub-type & Involved Parties (Two Mechanisms) & Real-world Attack &  Time & Victim Blockchains & Financial Loss & Defenses \\
%       \midrule
%       Permission Issue (PI) & Unchecked intermediary permission & $\mathbb{C}_S$ or $\mathbb{C}_D$ & PolyNetwork & 08/10/2021 & Ethereum & \$600 million & Au; BB\\\cmidrule{2-8}
%                 & Misused proof permission & $\mathbb{C}_S$ in step \ding{188} (Only Lock) & Plasma & 10/05/2021 & Polygon & \$850 million & BB \\
%                         && $\mathbb{C}_S$ or $\mathbb{C}_D$ & Binance Bridge & 10/06/2022 & BNB & \$566 million & BB; HF \\\cmidrule{2-8}
%                 & Problematic approval permission & $\mathbb{C}_S$ or $\mathbb{C}_D$ & Multichain & 01/18/2022 & Ethereum & \$3 million & UVC; RIA \\
%                                         &&& LI.FI & 05/20/2022 & Ethereum & \$0.6 million & UVC \\\cmidrule{2-8}
%                 & Invalid signature permission & $\mathbb{C}_D$ in step \ding{184} & ChainSwap & 07/10/2021 & Ethereum & \$8 million & Au; BB\\
%                              &&& Wormhole & 02/02/2022 & Solana; Ethereum & \$320 million & BB\\\cmidrule{2-8}
%                 & Leaked key permission & \BOS & WonderHero & 04/07/2022 & BNB & \$0.3 million & Au; UVC; BB\\ 
%                            &&& Ronin Network & 05/29/2022 & Ethereum & \$625 million & Au; IVD\\
%                            &&& Horizon Bridge & 06/24/2022 & Ethereum, BNB & \$100 million & Au\\
                           
%       % \addlinespace
%       \cmidrule{1-8}
%       Logic Issue (LI) & Incorrect balance logic & $\mathbb{C}_S$ or $\mathbb{C}_D$ & Polkabridge & 11/22/2021 & Ethereum & \$0.6 million & UVC \\
%                 & Inaccurate initialization logic & $\mathbb{C}_S$ or $\mathbb{C}_D$ & Nomad & 08/02/2022 & Moonbeam, Ethereum & \$190 million & BB\\
%       % \addlinespace
%       \cmidrule{1-8}
%       Event Issue (EI) & Incorrect event emission & $\mathbb{C}_S$ in step \ding{182} & Qubit & 01/27/2022 & Ethereum; BNB & \$80 million & BB\\
%                                     &&& Meter.io & 02/05/2022 & Ethereum; BNB; Moonriver & \$4.2 million & BB \\\cmidrule{2-8}
%                 & Fake event emission & \CS in step \ding{182} and \BOS in step \ding{183} & Cennznet & 05/08/2022 & Ethereum & \$0.4 million & UVC; EOS \\
%       \bottomrule
%     \end{tabular}
    
%     \caption{\small A taxonomy of cross-chain bridge attacks and vulnerabilities. 
%     Involved Parties (Two Mechanisms presented in~\secref{sec:pri:mec}): Lock means the Lock-and-Mint; Burn-and-Release mechanism.
%     % Involved Parties (Lock; Liquidity) represent the vulnerability involved parties and steps in the two mechanisms (presented in \secref{sec:pri:mec}) and N/A means the vulnerability cannot be exploited.
%     Defenses (presented in~\secref{sec:defense}): Au: Auditing; BB: Bug Bounty; HF: Hard Fork of Blockchain; UVC: Upgrading Vulnerable Contract; RIA: Revoking Infinite Approval; IVD: Increasing Validator Decentralization; EOS: Examining Off-chain Server.} 
%     \label{tbl:attack-class}
%     \vspace{-12pt}
% \end{table*}

% revised table
% \begin{table*}[t]
%     \centering
%     % \resizebox{0.95\linewidth}{!}{
%     % \scriptsize
%     \footnotesize
%     \begin{tabular}{lllllllll}
%       \toprule
%       Type & Sub-type & Involved Parties (Two Mechanisms) & Real-world Attack &  Time & Victim Blockchains & Financial Loss & Defenses \\
%       \midrule
%       PI & 4.1.1. PI1:Unchecked intermediary permission & $\mathbb{C}_S$ or $\mathbb{C}_D$ & PolyNetwork & 08/10/2021 & Ethereum & \$600 million & Au; BB\\\cmidrule{2-8}
%                 & 4.1.2. PI2:Misused proof permission & $\mathbb{C}_S$ in step \ding{188} (Only Lock) & Plasma & 10/05/2021 & Polygon & \$850 million & BB \\
%                         && $\mathbb{C}_S$ or $\mathbb{C}_D$ & Binance Bridge & 10/06/2022 & BNB & \$566 million & BB; HF \\\cmidrule{2-8}
%                 & 4.1.3. PI3:Problematic approval permission & $\mathbb{C}_S$ or $\mathbb{C}_D$ & Multichain & 01/18/2022 & Ethereum & \$3 million & UVC; RIA \\
%                                         &&& LI.FI & 05/20/2022 & Ethereum & \$0.6 million & UVC \\\cmidrule{2-8}
%                 & 4.1.4. PI4:Invalid signature permission & $\mathbb{C}_D$ in step \ding{184} & ChainSwap & 07/10/2021 & Ethereum & \$8 million & Au; BB\\
%                              &&& Wormhole & 02/02/2022 & Solana; Ethereum & \$320 million & BB\\\cmidrule{2-8}
%                 & 4.1.5. PI5:Leaked key permission & \BOS & WonderHero & 04/07/2022 & BNB & \$0.3 million & Au; UVC; BB\\ 
%                            &&& Ronin Network & 05/29/2022 & Ethereum & \$625 million & Au; IVD\\
%                            &&& Horizon Bridge & 06/24/2022 & Ethereum, BNB & \$100 million & Au\\
                           
%       % \addlinespace
%       \cmidrule{1-8}
%       LI & 4.2.1. LI1:Incorrect balance logic & $\mathbb{C}_S$ or $\mathbb{C}_D$ & Polkabridge & 11/22/2021 & Ethereum & \$0.6 million & UVC \\
%                 & 4.2.2. LI2:Inaccurate initialization logic & $\mathbb{C}_S$ or $\mathbb{C}_D$ & Nomad & 08/02/2022 & Moonbeam, Ethereum & \$190 million & BB\\
%       % \addlinespace
%       \cmidrule{1-8}
%       EI & 4.3.1. EI1:Incorrect event emission & $\mathbb{C}_S$ in step \ding{182} & Qubit & 01/27/2022 & Ethereum; BNB & \$80 million & BB\\
%                                     &&& Meter.io & 02/05/2022 & Ethereum; BNB; Moonriver & \$4.2 million & BB \\\cmidrule{2-8}
%                 & 4.3.2. EI2:Fake event emission & \CS in step \ding{182} and \BOS in step \ding{183} & Cennznet & 05/08/2022 & Ethereum & \$0.4 million & UVC; EOS \\
%       \bottomrule
%     \end{tabular}
    
%     \caption{\small A taxonomy of cross-chain bridge attacks and vulnerabilities. 
%     Type: PI: Permission Issue; LI: Logic Issue; EI: Event Issue.
%     Involved Parties (Two Mechanisms presented in~\secref{sec:pri:mec}): Lock: Lock-and-Mint; Burn-and-Release mechanism.
%     % Involved Parties (Lock; Liquidity) represent the vulnerability involved parties and steps in the two mechanisms (presented in \secref{sec:pri:mec}) and N/A means the vulnerability cannot be exploited.
%     Defenses (presented in~\secref{sec:defense}): Au: Auditing; BB: Bug Bounty; HF: Hard Fork of Blockchain; UVC: Upgrading Vulnerable Contract; RIA: Revoking Infinite Approval; IVD: Increasing Validator Decentralization; EOS: Examining Off-chain Server.} 
%     \label{tbl:attack-class}
%     \vspace{-12pt}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     % \resizebox{0.95\linewidth}{!}{
%     % \scriptsize
%     \footnotesize
%     \begin{tabular}{llllllllll}
%       \toprule
%       Type & Sub-type & Attack Surface & Identities & Real-world Attack &  Time & Victim Blockchains & Loss (\$million) & Defenses \\
%       \midrule
%       PI & 4.1.1. PI1:Unchecked intermediary permission & N/A & $\mathbb{C}_S$ or $\mathbb{C}_D$ & PolyNetwork & 08/10/2021 & Ethereum & 600.0 & Au; BB\\\cmidrule{2-9}
%                 & 4.1.2. PI2:Misused proof permission & A8 & $\mathbb{C}_S$ & Plasma & 10/05/2021 & Polygon & 850.0 & BB \\
%                         && A8 &$\mathbb{C}_S$ or $\mathbb{C}_D$ & Binance Bridge & 10/06/2022 & BNB & 566.0 & BB; HF \\\cmidrule{2-9}
%                 & 4.1.3. PI3:Problematic approval permission & N/A & $\mathbb{C}_S$ or $\mathbb{C}_D$ & Multichain & 01/18/2022 & Ethereum & 3.0 & UVC; RIA \\
%                                         &&&& LI.FI & 05/20/2022 & Ethereum & 0.6 & UVC \\\cmidrule{2-9}
%                 & 4.1.4. PI4:Invalid signature permission & A4 & $\mathbb{C}_D$ & ChainSwap & 07/10/2021 & Ethereum & 8.0 & Au; BB\\
%                              &&&& Wormhole & 02/02/2022 & Solana; Ethereum & 320.0 & BB\\\cmidrule{2-8}
%                 & 4.1.5. PI5:Leaked key permission & N/A & \BOS & WonderHero & 04/07/2022 & BNB & 0.3 & Au; UVC; BB\\ 
%                            &&&& Ronin Network & 05/29/2022 & Ethereum & 625.0 & Au; IVD\\
%                            &&&& Horizon Bridge & 06/24/2022 & Ethereum, BNB & 100.0 & Au\\
                           
%       % \addlinespace
%       \cmidrule{1-9}
%       LI & 4.2.1. LI1:Incorrect balance logic & N/A & $\mathbb{C}_S$ or $\mathbb{C}_D$ & Polkabridge & 11/22/2021 & Ethereum & \$0.6 million & UVC \\
%                 & 4.2.2. LI2:Inaccurate initialization logic & A13 & $\mathbb{C}_S$ or $\mathbb{C}_D$ & Nomad & 08/02/2022 & Moonbeam, Ethereum & \$190 million & BB\\
%       % \addlinespace
%       \cmidrule{1-8}
%       EI & 4.3.1. EI1:Incorrect event emission & A1 & $\mathbb{C}_S$ & Qubit & 01/27/2022 & Ethereum; BNB & \$80 million & BB\\
%                                     &&&& Meter.io & 02/05/2022 & Ethereum; BNB; Moonriver & \$4.2 million & BB \\\cmidrule{2-8}
%                 & 4.3.2. EI2:Fake event emission & A1 and A3 & \CS and \BOS & Cennznet & 05/08/2022 & Ethereum & \$0.4 million & UVC; EOS \\
%       \bottomrule
%     \end{tabular}
    
%     \caption{\small A taxonomy of cross-chain bridge attacks and vulnerabilities. 
%     Type: PI: Permission Issue; LI: Logic Issue; EI: Event Issue.
%     Involved Parties (Two Mechanisms presented in~\secref{sec:pri:mec}): Lock: Lock-and-Mint; Burn-and-Release mechanism.
%     % Involved Parties (Lock; Liquidity) represent the vulnerability involved parties and steps in the two mechanisms (presented in \secref{sec:pri:mec}) and N/A means the vulnerability cannot be exploited.
%     Defenses (presented in~\secref{sec:defense}): Au: Auditing; BB: Bug Bounty; HF: Hard Fork of Blockchain; UVC: Upgrading Vulnerable Contract; RIA: Revoking Infinite Approval; IVD: Increasing Validator Decentralization; EOS: Examining Off-chain Server.} 
%     \label{tbl:attack-class}
%     \vspace{-12pt}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     % \resizebox{0.95\linewidth}{!}{
%     % \scriptsize
%     \footnotesize
%     \begin{tabular}{lllllllll}
%       \toprule
%       Type & Sub-type & Attack Surface & Identities & Real-world Attack & Victim Blockchains & Loss (\$million) & Defenses \\
%       \midrule
%       PI & 4.1.1. PI1:Unchecked intermediary permission & N/A & $\mathbb{C}_S$ or $\mathbb{C}_D$ & 08/10/2021: PolyNetwork & Ethereum & 600.0 &  & Au; BB \\\cmidrule{2-8}
%                 & 4.1.2. PI2:Misused proof permission & A8 & $\mathbb{C}_S$ & 10/05/2021: Plasma & Polygon & 850.0 & BB \\
%                         && A8 &$\mathbb{C}_S$ or $\mathbb{C}_D$ & 10/06/2022: Binance Bridge & BNB & 566.0 & BB; HF \\\cmidrule{2-8}
%                 & 4.1.3. PI3:Problematic approval permission & N/A & $\mathbb{C}_S$ or $\mathbb{C}_D$ & 01/18/2022: Multichain & Ethereum & 3.0 & UVC; RIA \\
%                                         &&&& 05/20/2022: LI.FI & Ethereum & 0.6 & UVC \\\cmidrule{2-9}
%                 & 4.1.4. PI4:Invalid signature permission & A4 & $\mathbb{C}_D$ & 07/10/2021: ChainSwap & Ethereum & 8.0 & Au; BB\\
%                              &&&& 02/02/2022: Wormhole & Solana; Ethereum & 320.0 & BB\\\cmidrule{2-8}
%                 & 4.1.5. PI5:Leaked key permission & N/A & \BOS & 04/07/2022: WonderHero & BNB & 0.3 & Au; UVC; BB\\ 
%                            &&&& 05/29/2022: Ronin Network & Ethereum & 625.0 & Au; IVD\\
%                            &&&& 06/24/2022: Horizon Bridge & Ethereum, BNB & 100.0 & Au\\
                           
%       % \addlinespace
%       \cmidrule{1-8}
%       LI & 4.2.1. LI1:Incorrect balance logic & N/A & $\mathbb{C}_S$ or $\mathbb{C}_D$ & 11/22/2021: Polkabridge & Ethereum & \$0.6 million & UVC \\
%                 & 4.2.2. LI2:Inaccurate initialization logic & A13 & $\mathbb{C}_S$ or $\mathbb{C}_D$ & 08/02/2022: Nomad & Moonbeam, Ethereum & \$190 million & BB\\
%       % \addlinespace
%       \cmidrule{1-8}
%       EI & 4.3.1. EI1:Incorrect event emission & A1 & $\mathbb{C}_S$ & 01/27/2022: Qubit & Ethereum; BNB & \$80 million & BB\\
%                                     &&&& 02/05/2022: Meter.io & Ethereum; BNB; Moonriver & \$4.2 million & BB \\\cmidrule{2-8}
%                 & 4.3.2. EI2:Fake event emission & A1 and A3 & \CS and \BOS & 05/08/2022: Cennznet & Ethereum & \$0.4 million & UVC; EOS \\
%       \bottomrule
%     \end{tabular}
    
%     \caption{\small A taxonomy of cross-chain bridge attacks and vulnerabilities. 
%     Type: PI: Permission Issue; LI: Logic Issue; EI: Event Issue.
%     Involved Parties (Two Mechanisms presented in~\secref{sec:pri:mec}): Lock: Lock-and-Mint; Burn-and-Release mechanism.
%     % Involved Parties (Lock; Liquidity) represent the vulnerability involved parties and steps in the two mechanisms (presented in \secref{sec:pri:mec}) and N/A means the vulnerability cannot be exploited.
%     Defenses (presented in~\secref{sec:defense}): Au: Auditing; BB: Bug Bounty; HF: Hard Fork of Blockchain; UVC: Upgrading Vulnerable Contract; RIA: Revoking Infinite Approval; IVD: Increasing Validator Decentralization; EOS: Examining Off-chain Server.} 
%     \label{tbl:attack-class}
%     \vspace{-12pt}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     % \resizebox{0.95\linewidth}{!}{
%     % \scriptsize
%     \footnotesize
%     \begin{tabular}{llllllll}
%       \toprule
%       Type & Sub-type & Surface & Identities & Real-world Attack & Loss (\$million) & Defenses \\
%       \midrule
%       PI & 4.1.1. PI1:Unchecked intermediary permission & N/A & $\mathbb{C}_S$ or $\mathbb{C}_D$ & 08/10/2021: PolyNetwork & 600.0: Eth & Au; BB \\\cmidrule{2-7}
%                 & 4.1.2. PI2:Misused proof permission & A8 & $\mathbb{C}_S$ & 10/05/2021: Plasma & 850.0: Pol & BB \\
%                         && A8 &$\mathbb{C}_S$ or $\mathbb{C}_D$ & 10/06/2022: Binance Bridge & 566.0: Bnb & BB; HF \\\cmidrule{2-7}
%                 & 4.1.3. PI3:Problematic approval permission & N/A & $\mathbb{C}_S$ or $\mathbb{C}_D$ & 01/18/2022: Multichain & 3.0: Eth & UVC; RIA \\
%                                         &&&& 05/20/2022: LI.FI & 0.6: Eth & UVC \\\cmidrule{2-7}
%                 & 4.1.4. PI4:Invalid signature permission & A4 & $\mathbb{C}_D$ & 07/10/2021: ChainSwap & 8.0: Eth & Au; BB\\
%                              &&&& 02/02/2022: Wormhole & 320.0: Sol;Eth & BB\\\cmidrule{2-7}
%                 & 4.1.5. PI5:Leaked key permission & N/A & \BOS & 04/07/2022: WonderHero & 0.3: Bnb & Au; UVC; BB\\ 
%                            &&&& 05/29/2022: Ronin Network & 625.0: Eth& Au; IVD\\
%                            &&&& 06/24/2022: Horizon Bridge & 100.0: Eth;Bnb & Au\\
                           
%       % \addlinespace
%       \cmidrule{1-7}
%       LI & 4.2.1. LI1:Incorrect balance logic & N/A & $\mathbb{C}_S$ or $\mathbb{C}_D$ & 11/22/2021: Polkabridge & 0.6: Eth & UVC \\
%                 & 4.2.2. LI2:Inaccurate initialization logic & A13 & $\mathbb{C}_S$ or $\mathbb{C}_D$ & 08/02/2022: Nomad & 190.0: Mob;Eth & BB\\
%       % \addlinespace
%       \cmidrule{1-7}
%       EI & 4.3.1. EI1:Incorrect event emission & A1 & $\mathbb{C}_S$ & 01/27/2022: Qubit & 80.0: Eth;Bnb & BB\\
%                                     &&&& 02/05/2022: Meter.io & 4.2: Eth;Bnb;Mor & BB \\\cmidrule{2-7}
%                 & 4.3.2. EI2:Fake event emission & A1 and A3 & \CS and \BOS & 05/08/2022: Cennznet & 0.4: Eth& UVC; EOS \\
%       \bottomrule
%     \end{tabular}
    
%     \caption{\small A taxonomy of cross-chain bridge attacks and vulnerabilities. 
%     Type: PI: Permission Issue; LI: Logic Issue; EI: Event Issue.
%     Involved Parties (Two Mechanisms presented in~\secref{sec:pri:mec}): Lock: Lock-and-Mint; Burn-and-Release mechanism.
%     % Involved Parties (Lock; Liquidity) represent the vulnerability involved parties and steps in the two mechanisms (presented in \secref{sec:pri:mec}) and N/A means the vulnerability cannot be exploited.
%     Defenses (presented in~\secref{sec:defense}): Au: Auditing; BB: Bug Bounty; HF: Hard Fork of Blockchain; UVC: Upgrading Vulnerable Contract; RIA: Revoking Infinite Approval; IVD: Increasing Validator Decentralization; EOS: Examining Off-chain Server.} 
%     \label{tbl:attack-class}
%     \vspace{-12pt}
% \end{table*}


\begin{table*}[t]
    \centering
    % \resizebox{0.95\linewidth}{!}{
    % \scriptsize
    \footnotesize
    \begin{tabular}{llllll}
      \toprule
      Type & Sub-type & Attack Surface & Real-world Attack & Loss (\$million) & Defenses \\
      \midrule
      PI & Unchecked intermediary permission & A12($\mathbb{C}_S$ or $\mathbb{C}_D$) & 08/10/2021 PolyNetwork & 600:Eth & Au;BB \\\cmidrule{2-6}
                & Misused proof permission & A8($\mathbb{C}_S$) & 10/05/2021 Plasma & 850:Pol & BB \\
                        && A8($\mathbb{C}_S$ or $\mathbb{C}_D$) & 10/06/2022 Binance Bridge & 566:Bnb & BB;HF \\\cmidrule{2-6}
                & Problematic approval permission & A12($\mathbb{C}_S$ or $\mathbb{C}_D$) & 01/18/2022 Multichain & 3:Eth & UVC;RIA \\
                                        &&& 05/20/2022 LI.FI & 0.6:Eth & UVC \\\cmidrule{2-6}
                & Invalid signature permission & A4($\mathbb{C}_D$) & 07/10/2021 ChainSwap & 8:Eth & Au;BB\\
                             &&& 02/02/2022 Wormhole & 320:Sol;Eth & BB\\\cmidrule{2-6}
                & Leaked key permission & A10(\BOS) & 04/07/2022 WonderHero & 0.3:Bnb & Au;UVC;BB\\ 
                           &&& 05/29/2022 Ronin Network & 625:Eth& Au;IVD\\
                           &&& 06/24/2022 Horizon Bridge & 100:Eth;Bnb & Au\\\cmidrule{1-6}
                           
      % \addlinespace
      
      LI & Incorrect balance logic & A12($\mathbb{C}_S$ or $\mathbb{C}_D$) & 11/22/2021 Polkabridge & 0.6:Eth & UVC \\
                & Inaccurate initialization logic & A13($\mathbb{C}_S$ or $\mathbb{C}_D$) & 08/02/2022 Nomad & 190:Mob;Eth & BB\\
      % \addlinespace
      \cmidrule{1-6}
      EI & Incorrect event emission & A1($\mathbb{C}_S$) & 01/27/2022 Qubit & 80:Eth;Bnb & BB\\
                                    &&& 02/05/2022 Meter.io & 4.2:Eth;Bnb;Mor & BB \\\cmidrule{2-6}
                & Fake event emission & A1(\CS) and A3(\BOS) & 05/08/2022 Cennznet & 0.4:Eth& UVC;EOS \\
      \bottomrule
    \end{tabular}
    
    \caption{\small A taxonomy of cross-chain bridge attacks and vulnerabilities. 
    {\bf Type:} PI: Permission Issue; LI: Logic Issue; EI: Event Issue.
    {\bf Attack Surface:} $A_{i}$ (A1, A4, A8, A10, A12, A13) is the index of possible attacks defined in~\secref{sec:vuls}; \CS, \CD, and \BOS are involved identities in~\figref{figs:workflow}.
    {\bf Loss (\$million)}: total monetary loss, which also includes victim blockchains: Eth: Ethereum; Pol: Polygon; Bnb: BNB; Sol: Solana; Mob: Moonbeam; Mor: Moonriver. 
    {\bf Defenses} (presented in~\secref{sec:defense}): Au: Auditing; BB: Bug Bounty; HF: Hard Fork of Blockchain; UVC: Upgrading Vulnerable Contract; RIA: Revoking Infinite Approval; IVD: Increasing Validator Decentralization; EOS: Examining Off-chain Server.}
    % \xz{please revise caption after resolving N/A}
    \mz{need revision: Axxx}
    % \mz{revised a lot}\xz{What is N/A? why there is N/A? Is it not covered in the taxonomy?} \mz{not covered, since }
    \label{tbl:attack-class}
    \vspace{-12pt}
\end{table*}

==> 6-recommendations.tex <==
\section{Recommendations to Developers}
\label{sec:recom}
Based on our study, this section offers recommendations for developers building on-chain backends comprising smart contracts (for blockchain transactions) and off-chain servers (for off-chain operations).

\subsection{On-chain Backend}

\bheading{Ensuring proper permission-handling code.} Developers must thoroughly review all possible execution paths regarding permission checks. In addition, they can use tools such as Manticore~\cite{mossberg2019manticore} to assess code correctness.

\bheading{Avoiding unverified smart contract calls.} To prevent attacks where attackers deploy malicious smart contracts and hijack the control flow to their code, developers should avoid calling unverified smart contracts, particularly user-specified contracts, unless absolutely necessary.

\bheading{Checking return values of external calls.} Developers must be mindful of return values of functions, especially external function calls, as attackers can leverage inconsistencies caused by unchecked return values to launch exploits.

\bheading{Avoiding directly copying code.} While copying smart contract code from popular projects may save time, it can also result in code with bugs or vulnerabilities. Therefore, developers should closely examine the code and understand its logic.

\bheading{Setting longer withdraw latency.} Increasing the latency on token withdrawal can provide developers with additional time to mitigate risks. However, it may also affect bridge performance, and developers must weigh the trade-off between security and speed.

\bheading{Providing insurance.} Bridges can establish insurance for assets to compensate users in case of an attack, similar to real-world financial services. While precautions can reduce attack risks, insurance can mitigate users' financial losses in the event of an attack.


\subsection{Off-chain Server}

\bheading{Money monitoring.} 
DApps must vigilantly monitor their transactions to prevent losses from copycat or 1-day attacks. For instance, Ronin~\cite{ronin-attack} was aware of the attack several days after it occurred, avoiding further attacks. DApps must keep a close watch on transactions with unusual behaviors, such as large transfers or minting and burning of tokens. It is recommended to receive early alerts for such transactions.



